Non-Parallel Text Style Transfer with Self-Parallel Supervision

The performance of existing text style transfer models is severely limited by the non-parallel datasets on which the models are trained. In non-parallel datasets, no direct mapping exists between sentences of the source and target style; the style transfer models thus only receive weak supervision of the target sentences during training, which often leads the model to discard too much style-independent information, or utterly fail to transfer the style. In this work, we propose LaMer, a novel text style transfer framework based on large-scale language models. LaMer first mines the roughly parallel expressions in the non-parallel datasets with scene graphs, and then employs MLE training, followed by imitation learning refinement, to leverage the intrinsic parallelism within the data. On two benchmark tasks (sentiment & formality transfer) and a newly proposed challenging task (political stance transfer), our model achieves qualitative advances in transfer accuracy, content preservation, and fluency. Further empirical and human evaluations demonstrate that our model not only makes training more efficient, but also generates more readable and diverse expressions than previous models.

==> tables/data_stats.tex <==
\begin{table*}[!t]
\centering
\resizebox{0.92\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
\multicolumn{1}{c}{} &
  \multicolumn{2}{c}{\crule[RBRed]{0.15cm}{0.15cm}\ \textbf{Sentiment}} &
  \multicolumn{2}{c}{\crule[RBGreen]{0.15cm}{0.15cm}\ \textbf{Formality}} &
  \multicolumn{2}{c}{\crule[RBBlue]{0.15cm}{0.15cm}\ \textbf{Political Stance}} \\ \cmidrule(l){2-7} 
\textbf{Training Data (S-Emb. + SAS)} &
  \textit{positive} &
  \textit{negative} &
  \textit{formal} &
  \textit{informal} &
  \textit{liberal} &
  \textit{conservative} \\ \midrule
\# Sent Pairs                         & \multicolumn{2}{c}{553,430}     & \multicolumn{2}{c}{93,157}      & \multicolumn{2}{c}{36,307}      \\
\# Scene Entities                           & 742,136        & 777,839        & 145,731         & 133,779       & 194,032         & 272,071       \\
Avg. Sent Len                         & 7.32           & 7.58           & 11.52           & 11.05         & 19.39           & 24.75         \\
Avg. \# Scene Ent. / Sent                       & 1.34           & 1.41           & 1.56            & 1.44          & 5.34            & 7.49          \\
Avg. \# $\textrm{Scene Ent.}^{\textrm{src}\cap\textrm{tgt}}$ (vs. RD) &
  \multicolumn{2}{c}{0.95 (0.73)} &
  \multicolumn{2}{c}{0.49 (0.02)} &
  \multicolumn{2}{c}{0.96 (0.10)} \\
Avg. SAS (vs. RD)                     & \multicolumn{2}{c}{\dpboxred{0.72} (0.55)} & \multicolumn{2}{c}{\dpboxgreen{0.29} (0.01)} & \multicolumn{2}{c}{\dpboxblue{0.25} (0.01)} \\
 &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} &
  \multicolumn{1}{l}{} \\
\textbf{Human Reference}               &      \textit{positive}          &      \textit{negative}     &      \textit{formal}           &       \textit{informal}        &         \textit{liberal}        &      \textit{conservative}         \\ \midrule
\# Sent Pairs                         & \multicolumn{2}{c}{500}         & \multicolumn{2}{c}{1020}        & \multicolumn{2}{c}{525}         \\
\# Scene Entities                           & 964            & 905            & 1,467           & 1,388         & 2,915           & 3,012         \\
Avg. Sent Len                         & 9.90           & 9.80           & 10.9            & 9.35          & 10.30           & 11.19         \\
Avg. \# Scene Ent. / Sent                       & 1.93           & 1.81           & 1.44            & 1.36          & 5.58            & 5.76          \\
Avg. \# $\textrm{Scene Ent.}^{\textrm{src}\cap\textrm{tgt}}$ & \multicolumn{2}{c}{1.53}        & \multicolumn{2}{c}{0.55}        & \multicolumn{2}{c}{1.78}        \\
Avg. SAS & \multicolumn{2}{c}{\dpboxred{0.73}}        & \multicolumn{2}{c}{\dpboxgreen{0.29}}        & \multicolumn{2}{c}{\dpboxblue{0.30}}        \\ \bottomrule
\end{tabular}%
}
\caption{Data statistics of three TST tasks in this work: Sentiment, Formality, and Political Stance Transfer. We compare the S-Emb. + SAS aligned version data (the upper part), with the human-annotated reference file (the bottom part). Notice that after alignment, the SAS of training data becomes much closer to that of human reference, which demonstrates we successfully align the non-parallel data into parallel form (comparable to the human reference). Among the three TST datasets, we find the political stance TST has the longest sentence length (see Avg. Sent Len), and more scene entities involved on average (see Avg. \# Scene Ent. / Sent). Human written references also reveal similar statistics (see the lower part of the table), which will potentially increase the difficulty to have a entity-matched transfer. We thus consider the political stance TST is a more challenging task than the other two.}
\label{tab:data_stats}
\end{table*}

==> tables/tab_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table}[!h]
\centering
\caption{Ablation experiments on the contributions of sub-components (discussed in ) of \methodname{} imitation learning (IL). \redit{Removing all IL modules (MLE only) will cause severe drop in content preservation (BLEU).}}
\label{tab:il_ablation}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}lcccccc@{}}
\toprule
 & \multicolumn{2}{c}{\textbf{Sentiment}} & \multicolumn{2}{c}{\textbf{Formality}} & \multicolumn{2}{c}{\textbf{Political Stance}} \\ \cmidrule(l){2-7} 
Ablation on \methodname{} IL              & ACC  & BLEU & ACC  & BLEU & ACC  & BLEU \\ \midrule
IL ($d_{\textsc{Sem}}$ + $d_{\textrm{Order}}$ + $d_{\textrm{Exist}}$) & 97.0 & 34.1 & 76.5 & 39.2 & 93.4 & 18.5 \\
IL ($d_{\textsc{Sem}}$ +  $d_{\textrm{Order}}$)         & 95.5 ($\downarrow$1.5) & 34.4 ($\uparrow$0.3) & 74.7  ($\downarrow$1.8) & 37.7 ($\downarrow$1.5)& 93.2 ($\downarrow$0.2) & 15.8 ($\downarrow$2.7) \\
IL ($d_{\textsc{Sem}}$ + $d_{\textrm{Exist}}$)         & 96.5 ($\downarrow$0.5) & 33.9 ($\downarrow$0.2) & 72.6 ($\downarrow$3.9) & 34.1 ($\downarrow$5.1) & 92.7 ($\downarrow$0.7) & 17.1 ($\downarrow$1.4) \\
IL ($d_{\textsc{Sem}}$)            & 95.1 ($\downarrow$1.9) & 33.3 ($\downarrow$0.8) & 71.9 ($\downarrow$4.6) & 32.5 ($\downarrow$6.7) & 89.9 ($\downarrow$0.5) & 13.9 ($\downarrow$4.6) \\ \cmidrule(r){1-1}
No IL (MLE Only)               & 93.1 ($\downarrow$3.9) & 33.2 ($\downarrow$0.9) & 68.7 ($\downarrow$7.8) & 27.2 ($\downarrow$12.0) & 89.8 ($\downarrow$0.6) & 8.8 ($\downarrow$9.7)  \\ \bottomrule
\end{tabular}%
}
\end{table}
